Enabling New HDLs with Agents

Large Language Models (LLMs) based agents are transforming the programming language landscape by facilitating learning for beginners, enabling code generation, and optimizing documentation workflows. Hardware Description Languages (HDLs), with their smaller user community, stand to benefit significantly from the application of LLMs as tools for learning new HDLs. This paper investigates the challenges and solutions of enabling LLMs for HDLs, particularly for HDLs that LLMs have not been previously trained on. This work introduces HDLAgent, an AI agent optimized for LLMs with limited knowledge of various HDLs. It significantly enhances off-the-shelf LLMs.

==> acknowledgments.tex <==
\section*{Acknowledgments}

We like to thank the reviewers for their feedback on the
paper. Special thanks to Amir Roth for his invaluable help and feedback.
The authors gratefully acknowledge Michael Huang, Luigi Capodieci,
Andrea Di Blas, and Matthew Guthaus for their feedback on the
pruning infrastructure.  This work was supported in part by the National Science
Foundation under grants 0546819 and 720913; Special Research Grant from the
University of California, Santa Cruz; Sun OpenSPARC Center of Excellence at
UCSC; gifts from SUN, Altera, Xilinx, and ChipEDA.  Any opinions, findings, and
conclusions or recommendations expressed herein are those of the authors and do
not necessarily reflect the views of the NSF.


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> model.tex <==
\section{Characterization Methodology}
\label{sec:model}

enin

\subsection{Direct Thermal Measurement Infrastructure}
\label{sec:irsetup} 


 
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "paper"
%%% End: 

